On the Misspecification of Linear Assumptions in Synthetic Control

The synthetic control (SC) method is a popular approach for estimating treatment effects from observational panel data. It rests on a crucial assumption that we can write the treated unit as a linear combination of the untreated units. This linearity assumption, however, can be unlikely to hold in practice and, when violated, the resulting SC estimates are incorrect. In this paper we examine two questions: (1) How large can the misspecification error be? (2) How can we limit it? First, we provide theoretical bounds to quantify the misspecification error. The bounds are comforting: small misspecifications induce small errors. With these bounds in hand, we then develop new SC estimators that are specially designed to minimize misspecification error. The estimators are based on additional data about each unit, which is used to produce the SC weights. (For example, if the units are countries then the additional data might be demographic information about each.) We study our estimators on synthetic data; we find they produce more accurate causal estimates than standard synthetic controls. We then re-analyze the California tobacco-program data of the original SC paper, now including additional data from the US census about per-state demographics. Our estimators show that the observations in the pre-treatment period lie within the bounds of misspecification error, and that the observations post-treatment lie outside of those bounds. This is evidence that our SC methods have uncovered a true effect.

==> tex/2-backgroud.tex <==
\section{Synthetic Controls and Misspecification}\label{sec:background}


We review the assumptions behind synthetic controls, the fine-grained model of \citet{shi2022assumptions}, and formulate the problem of characterizing the misspecification error induced by violation of the assumptions.

\subsection{Panel Data and a Causal Question}
Consider a panel dataset containing outcome measurements $y_{jt}$ for units $j= 0, ..., J$ over time periods $t=0, ..., T$. Unit $j=0$ is the \textit{target}. It has received an intervention at time $T_0$ that may have affected its outcomes $y_{0t}$ for $t \geq T_0$. The remaining units are \textit{donors}. They did not received an intervention.

For each unit and period, define a pair of potential outcomes $(Y_{jt}, \widetilde{Y}_{jt})$, where $\widetilde{Y}_{jt}$ is the potential outcome of unit $j$ at time $t$ in the world where unit $j$ received an intervention at $T_0$, while $Y_{jt}$ is the potential outcome in a world with no intervention.
For $j=0$ and $t \geq T_0$,  $y_{jt} =\widetilde{Y}_{jt}$, otherwise, $y_{jt} = Y_{jt}$.
% Each observed outcome $y_{jt}$ corresponds to one of the potential outcomes,
%   \begin{equation*}
%     y_{jt} =
%     \begin{cases}
%       \widetilde{Y}_{jt}, & \text{if}\ j=0 \text{ and } t \geq T_0 \\
%       Y_{jt}, & \text{otherwise}.
%     \end{cases}
%  \end{equation*}

Our causal question is, what would the target counterfactual be, had the intervention not occurred? We would like to estimate $Y_{0t}$ for $t \geq T_0$.

% fold in 

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{fig/California-James-bound.pdf}
%     \caption{James-bound estimator on California vs other state, with the states demographics distributions as extra sources (age, sex, race). (left) Weights obtained by the James-bound estimator. Five states have non-zero weights. (right) Per-capita cigarette packs sales in California and synthetic California. The shaded error band is given by the James-bound $\pm 9.5$.  Synthetic California matches pre-intervention California. The true California tobacco consumption \textit{escapes} the error band after the intervention, indicating an effective anti-tobacco campaign even with potential misspecification.}
%     \label{fig:california_jamesbound}
% \end{figure}
% Synthetic control estimates the unobserved potential outcomes of the target ($Y_{0t}(0)$ with $t \geq T_0$) using a weighted combination of the observed potential outcomes of the controls units ($Y_{jt}(0)$ with $j\neq 0$).
% Synthetic control uses a weighted combination of the controls units' outcomes in order to estimate the potential outcomes of the target, had it not been treated.
\subsection{Synthetic Controls and their Assumptions}

Synthetic control methods estimate the counterfactual outcomes of the target $Y_{0t}, t \geq T_0$ with a weighted combination of the outcomes of the donors. The SC weights are fitted from the pre-intervention outcomes,
% Because it only uses potential outcomes under no intervention, we simplify the notations by using $Y_{jt}$ to denote $Y_{jt}(0)$.
% SC use the pre-intervention outcomes across unit  
\begin{align}
w = \argmin_{w \in \Delta^J} \sum^{T_0-1}_{t=0} \Bigl(y_{0t} - \sum_{j}{w}_j  y_{jt} \Bigr)^2.  \label{eq:estimator}
\end{align}
% We use these weights and control units' observed outcomes to approximate the treated unit's counterfactual in the post-intervention time periods. 

The validity of SC relies on two conditions: (1) During the pre-intervention period, the target's outcomes can be written as a weighted combination of the control units' outcomes. (2) The weighted combination from the pre-intervention period generalizes to the post-intervention period.
We formalize these two conditions as C1 and C2.
\begin{description}[leftmargin=0cm]
\item[C1. (Perfect Pre-intervention Fit)]
Before the intervention, the target's outcomes can be written as a convex combination of the donors' outcomes,
    \begin{equation*}
    \exists w \in \Delta^J,  \hspace{2em} Y_{0t} = \sum_j w_j Y_{jt}, \hspace{2em} \forall t < T_0 .\label{eq:sc-linear-pre}
    \end{equation*}
\end{description}


% \begin{enumerate}
%     \item[\textbf{A1}] During the pre-intervention period, when no unit is treated, the target can be written as a convex combination of the donors,
%     \begin{equation}
%     \exists w \in \Delta^J,  \forall t < T_0,\hspace{2em} y_{0t} = \sum_j w_j y_{jt}  .\label{eq:sc-linear-pre}
%     \end{equation}
% \end{enumerate}

\begin{description}[leftmargin=0cm]
\item[C2. (Generalization of the SC Weights)]
After the intervention, the target's counterfactual outcomes can be estimated by combining the donors' outcomes with the weights identified in A1,
    \begin{equation*}
    Y_{0t} = \sum_j w_j Y_{jt}, \hspace{2em} \forall t \geq T_0.\label{eq:sc-linear-post}
    \end{equation*}
\end{description}


\citet{abadie2010synthetic} directly assumes that C1 holds for some weights.
To justify C2, one sufficient condition is that the outcomes under no intervention are generated by a linear factor model \citep{bai2009panel, abadie2010synthetic, ben2021augmented,  ferman2021synthetic}. That is, 
\begin{equation}
    Y_{jt} = \mu_j ^\top \lambda_t + \epsilon_{jt}, \label{eq:linear_model}
\end{equation}
where $\mu_j$ is a unit-specific latent factor, $\lambda_t$ is a time-dependent factor, and $\epsilon_{jt}$ is random noise. 
% This linear factor model usually implies that any convex combination identified on the pre-intervention outcomes will induce the same convex combination on the factors, and so will generalize to the post-intervention outcomes, i.e., C2.

\begin{remark}\label{rm:linear}
To be precise, \citet{abadie2010synthetic} further assumes that $A:=\sum_{t < T_0} \lambda_t^\top \lambda_t$ is nonsingular. Consequently, once $Y_{0t} = \sum_j w_j Y_{jt}$ for $t<T_0$, the invertability of $A$ implies $\mu_0 = \sum_j w_j \mu_j$ (we intuitively ``invert'' the factor model). The target (as represented by its latent factor) is a convex combination of the other units.
Because the combination holds for the factors, it holds for the outcomes of all periods, i.e., C2 holds.
\end{remark}


% - shi+ dig into the assumptions by contemplating individuals
% - it posits the idea of a set of *invariant causes* they are correlated to the intervention through the correlation to the units. 
% - the outcome is dependent on them invariant aross units
% - but the distribution of confounding causes changes unit-to-unit



\subsection{A Fine-grained Model for SC}

It is unclear why the linear factor model in \cref{eq:linear_model} will hold in practice; \citet{shi2022assumptions} explores a justification. The authors notice that SC often considers large units composed of multiple individuals (states, countries) and aggregated outcomes that are averages of individual-level outcomes (per-capita cigarette consumption). Therefore, they propose a ``fine-grained" model of synthetic controls, which introduces individual-level variables. The variable $Y_{ijt}$ denotes individual $i$'s outcome in unit $j$ at time $t$ (their cigarette consumption at time $t$). The outcome of each unit $Y_{jt}$ is the average of the individual outcomes in the unit. 

Finally, the authors posit the idea of \emph{invariant causes}, which we denote as $x_{ijt}$. The invariant causes $x_{ijt}$ are individual-level variables that follow two invariance assumptions.
(1) When conditioned on the invariant causes, the individual-level outcomes do not depend on which unit the individual is from. This way, $x \mapsto \E{Y_{ijt} | x_{ijt}=x}$ is the same function for all $i$ and $j$; we write it $\E[t]{Y | x}$.
(2) The distribution of the invariant causes in each unit can change from unit to unit but remain the same across time. The distribution of invariant causes over the individuals in unit $j$ is denoted $x \mapsto p_j(x)$, with no dependence in $t$. 

With these individual-level variables, \citet{shi2022assumptions} shows that the unit-level outcomes are
\begin{align}
\E{Y_{jt}} = \int_x \E[t]{Y \mid x} p_{j}(x)~ \text{d}x \label{eq:shi}.
\end{align}
Further, if the distributions of invariant causes $p_j$ are \emph{discrete} and \emph{finite} then \cref{eq:shi} becomes a finite sum, \begin{align}
   \E{Y_{jt}} = \sum_{x_k} \underbrace{\E[t]{Y \mid x_k}}_{(\lambda_t)_k}\underbrace{p_j(x_k)}_{(\mu_j)_k} = \lambda_t ^\top \mu_j.
   \label{eq:shi-2}
\end{align}
Thus \Cref{eq:shi-2} justifies the linear model and provides  context about what the latent factors might represent. 

% %While the fine grained model enables a nonparametric formulation in \cref{eq:shi}, by assuming the causes are discrete and finite, we 
% \begin{remark}\label{rm:nonparametric}
% In order to obtain A1 and A2, \citet{shi2022assumptions} assume that the distributions of causes $p_j$ are \emph{discrete} and \emph{finite}. There is a finite number $N$ of causes\footnote{$N$ is called $|S|$ in \citet{shi2022assumptions}.} $x_1, ..., x_N$. By doing so, the integral in \cref{eq:shi} becomes a finite sum, and rewrites $$\E{Y_{jt}} = E_t ^\top P_j,$$ where  $(E_t)_k = \E[t]{Y \mid x_k}$ and $(P_j)_k = p_j(x_k)$ are $N$-dimensional vectors. We obtain a linear model again. \citet{shi2022assumptions} further assume that there is more than $N$ donors, call this number $D$. Then, the target's distribution $p_0$ is a vector of dimension $N<D$, it can be written as a linear combination of the donors $p_j$.
% While the non-parametric model is very general, the finite and discrete distribution assumption of this work implies that the target's distribution $p_0$ can be written as a linear combination of the other units $p_j$.

% \end{remark}

% \begin{remark}
% The fine-grained model in \cref{eq:shi} is more general than the linear model in \cref{eq:linear_model}.
% If we assume that all the individuals in unit $j$ have the same causes $\mu_j$ and the expected conditional individual-level outcome is a linear function of the causes,$\E{Y \mid x} = x^\top \lambda_t$, we can recover the linear model in \cref{eq:linear_model}. We have $p_j(x) = \mathds{1}(x = \mu_j)$ and $$\E{Y_{jt}} = \int_x \E[t]{Y \mid x} p_{j}(x) ~ \text{d}x  = \mu_j^\top \lambda_t.$$

% \end{remark}

%The assumptions in \citet{shi2022assumptions} are equally strong as the ones in \citet{abadie2010synthetic}.
% The fine-grained model helped us understand where the linearity in \cref{eq:linear_model} could come from, and it was able to provide context about what the latent factors might represent. Now, it can help us to understand how the synthetic control assumptions might be violated. 

%Based on this model, we will define misspecifications, derive error bounds and an estimators.

% \begin{remark}
% The fine-grained model in \cref{eq:shi} is more general than the linear model in \cref{eq:linear_model}.
% If we assume that all the individuals in unit $j$ have the same causes $\mu_j$ and the expected conditional individual-level outcome is a linear function of the causes,$\E{Y \mid x} = x^\top \lambda_t$, we can recover the linear model in \cref{eq:linear_model}. We have $p_j(x) = \mathds{1}(x = \mu_j)$ and $$\E{Y_{jt}} = \int_x \E[t]{Y \mid x} p_{j}(x) ~ \text{d}x  = \mu_j^\top \lambda_t.$$

% \end{remark}

% In order to prove synthetic control, Shi et.al make one assumption on this non-parametric formulation: p_j are discrete distribution over a finite number of causes x, and there is more donors than causes. Then, it is possible to write p_0 as a linear  combination as the p_j, that is the unit 0 itself (as represented by its latent factor), can be written as a linear combination of the other units.




